Stealthy Backdoors as Compression Artifacts

In a backdoor attack on a machine learning model, an adversary produces a model that performs well on normal inputs but outputs targeted misclassifications on inputs containing a small trigger pattern. Model compression is a widely-used approach for reducing the size of deep learning models without much accuracy loss, enabling resource-hungry models to be compressed for use on resource-constrained devices. In this paper, we study the risk that model compression could provide an opportunity for adversaries to inject stealthy backdoors. We design stealthy backdoor attacks such that the full-sized model released by adversaries appears to be free from backdoors (even when tested using state-of-the-art techniques), but when the model is compressed it exhibits highly effective backdoors. We show this can be done for two common model compression techniques -- model pruning and model quantization. Our findings demonstrate how an adversary may be able to hide a backdoor as a compression artifact, and show the importance of performing security tests on the models that will actually be deployed not their precompressed version.

==> 051_pruning_experiments.tex <==
\section{Pruning Experiments}

%\caption{\emph{Unstructured prune; last two layers; case-I:} The model accuracy and attack accuracy. Full-size models are trained with the loss function designed for Case-I. In the training, the last two layers are considered to be unstructuredly pruned and the pruning rate for each layer is $0.8$. The last two layers of each trained full-size model are then pruned with the same varying pruning rate ($100$ values, varying from $0$ to $0.99$ with a step of $0.01$) to generate a series of pruned models. The model accuracy on clean testing set (\emph{Acc on clean images)}, the model accuracy on the testing set consisting of trigger images (\emph{Acc on trigger images}), and the \emph{Attack Accuracy} on testing set consisting of trigger images whose ground truth labels are not the target attack class, of each pruned model are reported in the figures. }


%\caption{\emph{Unstructured prune; last two layers; Case-II:} The model accuracy and attack accuracy. Full-size models are trained with the loss function designed for Case-II. In the training, the last two layers are considered to be unstructuredly pruned and the pruning range for each layer is $[0.2, 0.8]$. The last two layers of each trained full-size model are then pruned with the same varying pruning rate ($100$ values, varying from $0$ to $0.99$ with a step of $0.01$) to generate a series of pruned models. The model accuracy on clean testing set (\emph{Acc on clean images)}, the model accuracy on the testing set consisting of trigger images (\emph{Acc on trigger images}), and the \emph{Attack Accuracy} on testing set consisting of trigger images whose ground truth labels are not the target attack class, of each pruned model are reported in the figures.  }






%\begin{table*}[]
%	\centering
%	\caption{Leverage Neural Cleanse (S\&P' 19) to detect backdoors; GTSRB; Pruning range of last layer: [0.3, 0.8]}
%	\begin{tabular}{c|ccccc}
%		\hline
%		& Clean & Backdoor & Strategy-A & Strategy-B & Strategy-C \\ \hline
%		VGG-16 & N / 1.724062 & C{[}1, 40{]} / 3.066658 & 
%		C[34, 40, 35] / 2.920916 & N / 1.768546 &  C[15, 1, 35, 34] /  2.440167 \\ \hline
%		ResNet-18 & N / 1.943922 & C1 / 3.469773 & C40 / 2.168372 & N /  1.332258 & N / 1.710380 \\ \hline
%		MobileNetV2 & N / 1.967194 & C1 / 3.514052 & N / 1.727840 & C[38, 40] / 2.333802 & N / 1.527135 \\ \hline
%	\end{tabular}%
%\end{table*}
%
%\begin{table*}[]
%	\centering
%	\caption{Leverage Neural Cleanse (S\&P' 19) to detect backdoors; GTSRB; Pruning range of last layer: [0.4, 0.8]}
%	\begin{tabular}{c|ccccc}
%		\hline
%		& Clean & Backdoor & Strategy-A & Strategy-B & Strategy-C \\ \hline
%		VGG-16 & N / 1.724062 & C{[}1, 40{]} / 3.066658 & 
%		C[40, 33-38, 1, 10] / 4.079987 & C[34, 35, 38] /  2.389294 &  N / 1.853378 \\ \hline
%		ResNet-18 & N / 1.943922 & C1 / 3.469773 &  & N / 1.369652 &  N / 1.792950 \\ \hline
%		MobileNetV2 & N / 1.967194 & C1 / 3.514052 & N / 1.922554 & C25 / 2.142527 & N / 1.464896 \\ \hline
%	\end{tabular}%
%\end{table*}

%\begin{table*}[]
%	\centering
%	\caption{Leverage Neural Cleanse (S\&P' 19) to detect backdoors; GTSRB; Attempt-A }
%	\begin{tabular}{c|ccccc}
%		\hline
%		& Clean & Backdoor & Strategy-A & Strategy-B & Strategy-C \\ \hline
%		VGG-16 & N / 1.724062 & C{[}1, 40{]} / 3.066658 & 
%		C[40, 10] / 2.043252 & C[34, 37-40] /  3.147727 &  C[34, 1, 33] / 3.536088 \\ \hline
%		ResNet-18 & N / 1.943922 & C1 / 3.469773 & N/ 1.524517 & C[35-38] / 2.381776 &  N / 1.684542 \\ \hline
%		MobileNetV2 & N / 1.967194 & C1 / 3.514052 & N / 1.785782 & N / 1.064868 & C38 / 2.045002 ] \\ \hline
%	\end{tabular}%
%\end{table*}








\begin{figure*}[]
	\centering
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_vgg_cifar10_vx_4.pdf}
		\caption{VGG-16; Strategy-A; CIFAR-10}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_resnet18_cifar10_vx_4.pdf}
		\caption{ResNet-18; Strategy-A; CIFAR-10}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_mobilenet_cifar10_vx_4.pdf}
		\caption{MobileNetV2; Strategy-A; CIFAR-10}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_vgg_cifar10_vx_5.pdf}
		\caption{VGG-16; Strategy-B; CIFAR-10}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_resnet18_cifar10_vx_5.pdf}
		\caption{ResNet-18; Strategy-B; CIFAR-10}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_mobilenet_cifar10_vx_5.pdf}
		\caption{MobileNetV2; Strategy-B; CIFAR-10}
		\label{}
	\end{subfigure}
%	\caption{\emph{Anomaly index per class reported by Neural Cleanse.}  Each row corresponds to the detection results on a model that is trained with a specified class set as the \textit{target class} of the backdoor attack. Because there is no anomaly index for the classes whose reconstructed L1 norms are greater than MAD, we set the anomaly indexes of those classes as 0.  }
%	\label{}
%\end{figure*}
%
%
%\begin{figure*}[]
%	\centering
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_vgg_gtsrb_vx_4.pdf}
		\caption{VGG-16; Strategy-A; GTSRB}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_resnet18_gtsrb_vx_4.pdf}
		\caption{ResNet-18; Strategy-A; GTSRB}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_mobilenet_gtsrb_vx_4.pdf}
		\caption{MobileNetV2; Strategy-A; GTSRB}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_vgg_gtsrb_vx_5.pdf}
		\caption{VGG-16; Strategy-B; GTSRB}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_resnet18_gtsrb_vx_5.pdf}
		\caption{ResNet-18; Strategy-B; GTSRB}
		\label{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{fig/neural_cleanse_pruning_travel_all_labels/travel_all_labels_mobilenet_gtsrb_vx_5.pdf}
		\caption{MobileNetV2; Strategy-B; GTSRB}
		\label{}
	\end{subfigure}
	\caption{\emph{Anomaly index per class reported by Neural Cleanse.}  Each row corresponds to the detection results on a model that is trained with a specified class set as the \textit{target class} of the backdoor attack. Because there is no anomaly index for the classes whose reconstructed L1 norms are greater than MAD, we set the anomaly indexes of those classes as 0.  }
	\label{}
\end{figure*}




%\begin{figure*}[ht]
%	\centering
%	\begin{subfigure}[b]{0.48\textwidth}
%		\centering
%		\includegraphics[width=1\textwidth]{fig/pruning_nueral_cleanse/vgg_cifar_10.pdf}
%		\caption{VGG-16; CIFAR-10}
%		\label{fig:pruning_auto_compress_structured_gtsrb_b}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.48\textwidth}
%		\centering
%		\includegraphics[width=1\textwidth]{fig/pruning_nueral_cleanse/resnet18_cifar_10}
%		\caption{ResNet-18; GTSRB}
%		\label{fig:pruning_auto_compress_structured_gtsrb_a}
%	\end{subfigure}
%	\caption{\emph{L1 norm of the reconstructed trigger pattern} }
%	\label{fig:pruning_auto_compress_structured_gtsrb}
%\end{figure*}
%
%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=0.48\textwidth]{fig/pruning_nueral_cleanse/resnet18_gtsrb}
%	\caption{VGG-16; Strategy-C; GTSRB}
%	\label{fig:pruning_auto_compress_structured_gtsrb_c}
%\end{figure}


